State-Based Confidence Bounds for Data-Driven Stochastic Reachability Using Hilbert Space Embeddings

In this paper, we compute finite sample bounds for data-driven approximations of the solution to stochastic reachability problems. Our approach uses a nonparametric technique known as kernel distribution embeddings, and provides probabilistic assurances of safety for stochastic systems in a model-free manner. By implicitly embedding the stochastic kernel of a Markov control process in a reproducing kernel Hilbert space, we can approximate the safety probabilities for stochastic systems with arbitrary stochastic disturbances as simple matrix operations and inner products. We present finite sample bounds for point-based approximations of the safety probabilities through construction of probabilistic confidence bounds that are state- and input-dependent. One advantage of this approach is that the bounds are responsive to non-uniformly sampled data, meaning that tighter bounds are feasible in regions of the state- and input-space with more observations. We numerically evaluate the approach, and demonstrate its efficacy on a neural network-controlled pendulum system.

==> changes.tex <==
Fixed label of figure 3. 

==> coverletter.tex <==
Dear Prof. Petersen, 

We are submitting our revision to Automatica 20-1356, now titled, "State-Based Confidence Bounds for Data-DrivenStochastic Reachability Using Hilbert Space Embeddings," by Adam Thorpe, Kendric Ortiz, and Meeko Oishi.  

We have carefully considered the feedback from the Associate Editor and the reviewers, and have modified our manuscript accordingly.  A detailed description of our changes is described in the Response to Reviewers.  Major changes include 
1) reformulation of the title, abstract, and introduction to reflect a focus on the construction of state-based confidence bounds for data-driven stochastic reachability, 
2) inclusion of new technical content regarding reproducing kernal Hilbert spaces, and the distinction between point-based and set-based stochastic reachability, to ensure that the paper is self-contained, 
3) revised confidence bounds that are explicitly tied to the sample size, and 
4) revision of several technical points raised by the reviewers, including scalability, time horizons, and clarification of the sampling process. 

Thank you for your consideration. 

Sincerely, 
Meeko Oishi



---------------


In this paper, we compute finite sample bounds for data-driven
approximations of the solution to stochastic reachability problems. 
Our approach uses a nonparametric technique known as kernel
distribution embeddings, and provides probabilistic assurances of
safety for stochastic systems in a model-free manner.  By implicitly
embedding the stochastic kernel of a Markov control process in a
reproducing kernel Hilbert space, we can approximate the safety
probabilities for stochastic systems with arbitrary stochastic
disturbances as simple matrix operations and inner products.  We
present finite sample bounds for point-based approximations of the
safety probabilities through construction of probabilistic confidence
bounds that are state- and input-dependent. One advantage of this
approach is that the bounds are responsive to non-uniformly sampled
data, meaning that tighter bounds are feasible in regions of the state-
and input-space with more observations.  We numerically evaluate the
approach, and demonstrate its efficacy on a neural network-controlled
pendulum system.
